(Leftmost-Outermost) Beta Reduction is Invariant, Indeed

Slot and van Emde Boas' weak invariance thesis states that reasonable machines can simulate each other within a polynomially overhead in time. Is lambda-calculus a reasonable machine? Is there a way to measure the computational complexity of a lambda-term? This paper presents the first complete positive answer to this long-standing problem. Moreover, our answer is completely machine-independent and based over a standard notion in the theory of lambda-calculus: the length of a leftmost-outermost derivation to normal form is an invariant cost model. Such a theorem cannot be proved by directly relating lambda-calculus with Turing machines or random access machines, because of the size explosion problem: there are terms that in a linear number of steps produce an exponentially long output. The first step towards the solution is to shift to a notion of evaluation for which the length and the size of the output are linearly related. This is done by adopting the linear substitution calculus (LSC), a calculus of explicit substitutions modeled after linear logic proof nets and admitting a decomposition of leftmost-outermost derivations with the desired property. Thus, the LSC is invariant with respect to, say, random access machines. The second step is to show that LSC is invariant with respect to the lambda-calculus. The size explosion problem seems to imply that this is not possible: having the same notions of normal form, evaluation in the LSC is exponentially longer than in the lambda-calculus. We solve such an impasse by introducing a new form of shared normal form and shared reduction, deemed useful. Useful evaluation avoids those steps that only unshare the output without contributing to beta-redexes, i.e. the steps that cause the blow-up in size. The main technical contribution of the paper is indeed the definition of useful reductions and the thorough analysis of their properties.

==> lambda.tex <==
% !TEX root = main.tex
\section{Rewriting}
For us, an \emph{(abstract) reduction system} is a pair $(T, \str)$ consisting of
a set $T$ of terms and a binary relation $\str$ on $T$ called a
\emph{reduction (relation)}. When $(\tm,\tmtwo) \in \str$ we write
$\tm \str \tmtwo$ and we say that $\tm$ \emph{$\R$-reduces} to
$\tmtwo$. The reflexive and transitive closure of $\str$ is written
$\Rewn{\R}$. Composition of relations is denoted by juxtaposition.
Given $k \geq 0$, we write $a \Rew{\R}^k b$ iff $a$ is $\R$-related to
$b$ in $k$ steps, \ie\ $a \Rew{\R}^0 b$ if $a=b$ and $a \Rew{\R}^{k+1}
b$ if $\exists\ c$ such that  $a \str c$ and $c \Rew{\R}^k b$.

A term $\tm \in R$ is a \emph{$\R$-normal form} if there is no
$\tmtwo\in R$ such that $\tm\str \tmtwo$. Given a deterministic
reduction system $(T, \str)$, and a term $\tm \in T$, the expression
$\nos{\str}{\tm}$ stands for the number of reduction steps necessary
to reach the $\str$-normal form of $\tm$ along $\str$, or $\infty$ if
 $\tm$ diverges. Similarly, given a natural number $n$, the expression
$\strp{\str}{n}{\tm}$ stands for the term $\tmtwo$ such that
$\tm\str^n\tmtwo$, if $n\leq\nos{\str}{\tm}$, or for the normal form
of $\tm$ otherwise.


\section{\texorpdfstring{$\l$}{lambda}-Calculus}
\subsection{Statics}
The syntax of the $\l$-calculus is given by the following grammar for
terms:
$$
\tm,\tmtwo,\tmthree,\tmfour\grameq\var\midd \l \var. \tm \midd \tm \tmtwo.
$$ 
We use $\tm\isub{\var}{\tmtwo}$ for the usual (meta-level)
notion of substitution. An abstraction $\l
\var. \tm$ binds $\var$ in $\tm$, and we
silently work modulo $\alpha$-equivalence of these bound variables,
\eg\ $(\la\vartwo(\var\vartwo))\isub\var\vartwo =
\la\varthree(\vartwo\varthree)$. We use $\fv\tm$ for the set of
free variables of $\tm$.

\emph{Contexts.} One-hole contexts are defined by:
$$
\gctx \grameq \ctxhole\midd \l \var. \gctx\midd \ap\gctx \tm \midd\ap\tm\gctx,
$$ 
and the plugging of a term $\tm$ into a context $\gctx$ is defined by
\[\begin{array}{cccccccccccc}
   \ctxhole\ctxholep\tm & \defeq & \tm &&& (\gctx \tmtwo)\ctxholep\tm & \defeq & \gctx\ctxholep\tm \tmtwo\\
   (\l\var.\gctx)\ctxholep\tm & \defeq & \l\var.\gctx\ctxholep\tm &&& (\tmtwo \gctx)\ctxholep\tm & \defeq &  \tmtwo \gctx\ctxholep\tm
  \end{array}\]
As usual, plugging in a context can capture variables,
\eg\ $(\la\vartwo(\ctxhole\vartwo))\ctxholep\vartwo =
\la\vartwo(\vartwo\vartwo)$. The plugging $\gctxp\gctxtwo$ of a
context $\gctxtwo$ into a context $\gctx$ is defined analogously. Plugging will be implicitly extended to all notions of contexts in the paper, always in the expected way.


\subsection{Dynamics}
We define $\beta$-reduction $\tob$ as follows:
$$\begin{array}{c@{\hspace{1.5cm}}c}
  \textsc{Rule at Top Level} & \textsc{Contextual closure} \\
	(\l\var.\tm)\tmtwo \rtob \tm\isub\var\tmtwo &
        \gctxp \tm \tob \gctxp \tmtwo \textrm{~~~if } \tm \rtob \tmtwo \\
\end{array}$$
The \emph{position} of a $\beta$-redex $\gctxp \tm \tob \gctxp \tmtwo$ is the context $\gctx$ in which it takes place. To ease the language, we will identify a redex with its position. A \deff{derivation} $\deriv:\tm\to^k\tmtwo$
is a finite, possibly empty, sequence of reduction steps, sometimes given as
$\gctx_1;\ldots; \gctx_k$, \ie\ as the sequence of positions of reduced
redexes. We write $\size\tm$ for the size of $\tm$ and $\size\deriv$ for the length of
$\deriv$. \medskip




\emph{Leftmost-Outermost Derivations.} 
The left-to-right outside-in order on redexes is expressed as an order
on positions, \ie\ contexts. Let us warn the reader about a possible
source of confusion. The \emph{left-to-right outside-in} order in the
next definition is sometimes simply called \emph{left-to-right} (or
simply \emph{left}) order. The former terminology is used when terms
are seen as trees (where the left-to-right and the outside-in orders
are disjoint), while the latter terminology is used when terms are
seen as strings (where left-to-right is a total order). While the
study of standardization for the \lsc~\cite{non-standard-preprint}
uses the string approach (and thus only talks about the
\emph{left-to-right} order and the \emph{leftmost} redex), here some
of the proofs require
a delicate analysis of the relative positions of redexes and so we
prefer the more informative tree approach and define the order
formally.

\begin{definition}\hfill
  \begin{varenumerate}
  \item 
    The \deff{outside-in order}: 
    \begin{varvarenumerate}
    \item 
      \emph{Root}: $\ctxhole\outin\gctx$ for every context
      $\gctx\neq\ctxhole$;
    \item 
      \emph{Contextual closure}: If $\gctx\outin\gctxtwo$ then
      $\gctxthreep\gctx\outin\gctxthreep\gctxtwo$ for any context
      $\gctxthree$.
    \end{varvarenumerate}    
  \item 
    The \deff{left-to-right order}: $\gctx\leftright\gctxtwo$ is defined by:
    \begin{varvarenumerate}
    \item 
      \emph{Application}: If $\gctx\prefix \tm$ and
      $\gctxtwo\prefix\tmtwo$ then
      $\ap\gctx\tmtwo\leftright\ap\tm\gctxtwo$;
    \item 
      \emph{Contextual closure}: If $\gctx\leftright\gctxtwo$ then
      $\gctxthreep\gctx\leftright\gctxthreep\gctxtwo$ for any context
      $\gctxthree$.
    \end{varvarenumerate}  
  \item 
    The \deff{left-to-right outside-in order}:
    $\gctx\leftout\gctxtwo$ if $\gctx\outin\gctxtwo$ or
    $\gctx\leftright\gctxtwo$:
  \end{varenumerate}
\end{definition}

The following are a few examples. For every context $\gctx$, it holds
that $\ctxhole\not\leftright\gctx$. Moreover,
\begin{align*}
  \ap{(\l\var.\ctxhole)}\tm
  &\outin 
  \ap{(\l\var.(\ap{\ctxhole}\tmtwo)})\tm;\\
  \ap{(\ap\ctxhole\tm)}\tmtwo
  &\leftright
  \ap{(\ap\tmthree\tm)}\ctxhole.
\end{align*}

\begin{definition}[\lo\ $\beta$-Reduction]
  Let $\tm$ be a $\l$-term and $\gctx$ a redex of $\tm$. $\gctx$ is the \deff{leftmost-outermost}  $\beta$-redex (\lob\ for short) of $\tm$ 
   if $\gctx\leftout\gctxtwo$ for
  every other $\beta$-redex $\gctxtwo$ of $\tm$. We
  write $\tm\toblo\tmtwo$ if a step reduces
  the \lo\ $\beta$-redex.
\end{definition}

\subsection{Inductive \lob\ Contexts} It is useful to have an inductive characterization of the contexts in which $\toblo$ takes place. We use the following terminology: a term is \emph{neutral} if it is $\beta$-normal and it is not of the form $\la\var\tmtwo$, \ie\ it is not an abstraction. 
 
 \begin{definition}[\ilob\ Context]
 \label{def:ilob-ctx}
 Inductive \lob\ (or \ilob) contexts are defined by induction as follows:
 \begin{center}
$\begin{array}{cccccc}
	\AxiomC{}
	\RightLabel{(ax-\ilob)}
	\UnaryInfC{$\ctxhole$ is \ilob}
	\DisplayProof
	&
	\AxiomC{$\gctx$ is \ilob}
	\AxiomC{$\gctx\neq\la\var\gctxtwo$}
	\RightLabel{(@l-\ilob)}
	\BinaryInfC{$\gctx \tm$ is \ilob}
	\DisplayProof \\\\
	
	\AxiomC{$\gctx$ is \ilob}
	\RightLabel{($\l$-\ilob)}
	\UnaryInfC{$\la\var\gctx$ is \ilob}
	\DisplayProof &

	  \AxiomC{$\tm$ is neutral}
	\AxiomC{$\gctx$ is \ilob}
	\RightLabel{(@r-\ilob)}
	\BinaryInfC{$\tm \gctx$ is \ilob}
	\DisplayProof 
\end{array}$
\end{center}
 \end{definition}

As expected,

\begin{lemma}[$\toblo$-steps are Inductively \lob]
\label{l:toblo-ilob}
Let $\tm$ be a $\l$-term and $\gctx$ a redex in $\tm$. $\gctx$ is the \lob\ redex in $\tm$ iff $\gctx$ is \ilob.
\end{lemma}

\begin{proof}
  The left-to-right implication is by induction on $\gctx$.  The
  right-to-left implication is by induction on the definition of
  \emph{$\gctx$ is \ilob}.
\end{proof}


==> new-normal-form.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Normal Form Property}
\label{sect:normal-form}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 To show the normal form property we first have to generalize it to the relative unfolding in a context, in the next lemma, and then obtain it as a corollary. 
 
 
   The statement of the lemma essentially says that for a useful normal form $\tmtwo$ in a context $\ctx$ the unfolding $\relunf\tmtwo\ctx$ either unfolds to a $\tob$-normal form or it has a useful substitution redex provided by $\ctx$. The second case is stated in a more technical way, spelling out the components of the redex, and will be used twice later on, in \reflemma{loudb-are-ilou} in \refsect{new-projection} (page \pageref{l:loudb-are-ilou}) and \refprop{local-bound} in \refsect{nested} (page \pageref{prop:local-bound}). To have a simpler look at the statement we suggest to ignore cases \ref{p:nf-charac-dupl} and \ref{p:nf-charac-creation} at a first reading.

   
   
%\blue{
\begin{lemma}[Contextual Normal Form Property]
\label{l:nf-charac}
Let $\ctxp\tmtwo$ be such that $\tmtwo$ is a useful normal form and $\ctx$ is a shallow context. Then either
\begin{varenumerate}
	\item $\relunf\tmtwo\ctx$ is a $\beta$-normal form, or
	\item $\ctx\neq \ctxhole$ and there exists a shallow context $\ctxtwo$ such that 
	\begin{varvarenumerate}
		\item $\tmtwo = \ctxtwop\var$, and
		\item $\ctxp\ctxtwo$ is the position of a useful $\ls$-redex of $\ctxp\tmtwo$, namely
		\begin{varvarvarenumerate}
			\item \label{p:nf-charac-dupl}\emph{Relative Duplication}: $\relunf\var{\ctxp\ctxtwo}$ has a $\beta$-redex, or
			\item \label{p:nf-charac-creation}\emph{Relative Creation}: $\ctxtwo$ is applicative and $\relunf\var{\ctxp\ctxtwo}$ is an abstraction.
		\end{varvarvarenumerate}
	\end{varvarenumerate}
\end{varenumerate}
\end{lemma}

\begin{proof}
	Note that:
	\begin{varitemize}
		\item If there exists $\ctxtwo$ as in case 2 then $\ctx \neq \ctxhole$, otherwise case \ref{p:nf-charac-dupl} or case \ref{p:nf-charac-creation} would imply a useful substitution redex in $\tmtwo$, while $\tmtwo$ is a useful normal form by hypothesis.
		\item
                  Cases 1 and 2 are mutually exclusive: if \ref{p:nf-charac-dupl} or \ref{p:nf-charac-creation} holds clearly $\relunf\tmtwo\ctx$ has a $\beta$-redex. We are only left to prove that one of the two always holds.
	\end{varitemize}
	By induction on $\tmtwo$. Cases:
	\begin{varenumerate}
		\item \emph{Variable} $\tmtwo = \var$. If $\relunf\var\ctx$ is a $\beta$-normal form nothing remains to be shown. Otherwise, $\relunf\var{\ctx}$ has a $\beta$-redex and we are in case \ref{p:nf-charac-dupl}, setting $\ctxtwo \defeq \ctxhole$ (giving $\relunf\var{\ctxp\ctxtwo}= \relunf\var{\ctx}$).
		
	\item \emph{Abstraction} $\tmtwo = \la\vartwo\tmthree$. Follows from the \ih\ applied to $\tmthree$ and $\la\var\ctxhole$.
	
	\item \emph{Application} $\tmtwo = \tmthree\tmfour$. Note that $\relunf\tmtwo\ctx =_{\reflemmaeqp{relunf-prop}{zero}} \relunf\tmthree\ctx \relunf\tmfour\ctx$ and that $\tmthree$ is a useful normal form, since $\tmtwo$ is. We can then apply the \ih\ to $\tmthree$ and $\ctxp{\ctxhole\tmfour}$. There are two cases:
	\begin{varvarenumerate}
		\item \emph{$\relunf\tmthree{\ctxp{\ctxhole\tmfour}} = \relunf{\tmthree}{\ctx}$ is a normal form}. Sub-cases:
		\begin{varvarvarenumerate}
			\item \emph{$\relunf{\tmthree}{\ctx}$ is an abstraction $\la\vartwo\tmfive$}. This is the interesting inductive case, because it is the only one where the \ih\ provides case 1 for $\tmthree$ but the case ends proving case 2, actually \ref{p:nf-charac-creation}, for $\tmtwo$. In the other cases of the proof (3(a)ii, 3(b), and 4), instead, the case of the statement provided by the \ih\ is simply propagated \emph{mutatis mutandis}.
			
			Note that $\tmthree$ cannot have the form $\sctxp{\la\vartwo\tmsix}$, because otherwise $\tmtwo$ would not be $\tolou$ normal. Then it follows that $\tmthree = \sctxp\var$ (as $\tmthree$ cannot be an application). For the same reason, $\unf\tmthree$ cannot have the form $\la\vartwo\tmsix$. Then $\unf\tmthree = \varthree$ for some variable $\varthree$ (possibly $\varthree=\var$).  Now take $\ctxtwo \defeq \sctx \tmfour$.  Note that  $\ctxtwo$ is applicative and that $\relunf\var{\ctxp{\sctx \tmfour}} =_{\reflemmaeqp{relunf-prop}{four}} \relunf{\sctxp\var}{\ctxp{\ctxhole\tmfour}} = \relunf{\sctxp\var}{\ctx} = \relunf\tmthree\ctx = \la\vartwo\tmfive$. So we are in case \ref{p:nf-charac-creation} and there is a useful $\tols$-redex of position $\ctxp\ctxtwo$.			
			

			\item \emph{$\tmthree$ is not an abstraction}. Note that $\relunf\tmthree\ctx$ is neutral. Then the statement follows from the \ih\ applied to $\tmfour$ and $\ctxp{\tmthree\ctxhole}$. Indeed, if $\relunf\tmfour{\ctxp{\tmthree\ctxhole}} = \relunf\tmfour{\ctx}$ is a $\beta$-normal form then $\relunf\tmtwo\ctx = \relunf\tmthree\ctx \relunf\tmfour\ctx$ is a $\beta$-normal form and we are in case 1. While if exists $\ctxthree$ such that  $\tmfour = \ctxthreep\var$ verifies case 2 (with respect to $\ctxp{\tmthree\ctxhole}$) then $\ctxtwo \defeq \tmthree\ctxthree$ verifies case 2 with respect to $\ctx$.
		\end{varvarvarenumerate}
		
		\item \emph{exists $\ctxthree$ such that $\tmthree =\ctxthreep\var$ verifying case 2 of the statement with respect to $\ctxp{\ctxhole\tmfour}$}. Then case 2 holds for $\ctxtwo \defeq \ctxthree\tmfour$ with respect to $\ctx$.
	\end{varvarenumerate}
	
	\item \emph{Substitution} $\tmtwo = \tmthree\esub\vartwo\tmfour$. Note that $\relunf\tmtwo\ctx = \relunf{\tmthree\esub\vartwo\tmfour}{\ctx}=_{\reflemmaeqp{relunf-prop}{four}} \relunf{\tmthree}{\ctxp{\ctxhole\esub\vartwo\tmfour}}$. So we can apply the \ih\ to $\tmthree$ and $\ctxp{\ctxhole\esub\vartwo\tmfour}$, from which the statement follows.
	\end{varenumerate}
\end{proof}
%}


\begin{corollary}[Normal Form Property]
\label{coro:normal-form}
Let $\tm$ be a useful normal form. Then $\unf\tm$ is a $\beta$-normal form.
\end{corollary}

\begin{proof}
Let us apply \reflemma{nf-charac} to $\ctx \defeq \ctxhole$ and $\tmtwo \defeq \tm$. Since $\ctx = \ctxhole$, case 2 cannot hold, so that $\relunf\tm\ctx = \unf\tm$ is a $\beta$-normal form.
\end{proof}
\ben{At the end of the next section we will obtain the converse implication (\refcorollaryp{converse-prop-high-lev}{normal}), as a corollary of the strong projection property.}

\ben{Let us close this section with a comment. The auxiliary lemma for the normal form property is of a technical nature. Actually, it is a strong improvement (inspired by \cite{usef-constr}) over the sequence of lemmas we provided in the technical report \cite{EV}, that followed a different (worse) proof strategy. At a first reading the lemma looks very complex and it is legitimate to suspect that we did not fully understand the property we proved. We doubt, however, the existence of a much simpler proof, and believe that---despite the technical nature---our proof is compact. There seems to be an inherent difficulty given by the fact that useful reduction is a global notion, in the sense that it is not a rewriting rule closed by evaluation contexts, but it is defined by looking at the whole term at once. Its global character seems to prevent a simpler proof.}
 


==> new-projection.tex <==
% !TEX root = main.tex
\section{The Projection Property}
\label{sect:new-projection}
We now turn to the proof of the projection property. We already know that a single shallow $\db$-step projects to a single $\beta$-step (\reflemma{db-projection}). Therefore it remains to be shown that $\tolou$ $\db$-steps project on \lob\ steps. We do it contextually, in three steps: 

\begin{varenumerate}
	\item giving a (non-inductive) notion of \lou\ \emph{context}, and proving that if a redex $\ctx$ is a $\tolou$ redex then $\ctx$ is a \lou\ context.
	\item providing that \lou\ contexts admit a \emph{inductive} formulation.
	\item proving that \emph{inductive} \lou\ contexts unfold to inductive \lob\ contexts, that is where \lob\ steps take place.
\end{varenumerate}

As for the normal form property, the proof strategy is inspired by \cite{usef-constr}, and improves the previous proof in the technical report \cite{EV}.

\subsection{\lou\ Contexts} Remember that a term is \emph{neutral} if it is $\beta$-normal and is not of the form $\la\var\tmtwo$ (\ie\ it is not an abstraction). 

 \begin{definition}[\lou\ Contexts]
 \
  A context $\ctx$ is \lou\ if 
    \begin{varenumerate}
     	\item \emph{Leftmost}: whenever $\ctx = \ctxtwop{\tm\ctxthree}$ then $\relunf\tm\ctxtwo$ is neutral, and
			\item \emph{Outermost}: whenever $\ctx = \ctxtwop{\la\var\ctxthree}$ then $\ctxtwo$ is not applicative.
		\end{varenumerate}
	\end{definition}

The next lemma shows that $\tolou$ redexes take place in \lou\ contexts. In the last sub-case the proof uses the generalized form of the normal form property (\reflemma{nf-charac}).

\begin{lemma}[The Position of a $\tolou$\ Step is a \lou\ Context]
\label{l:loudb-are-ilou}
Let $\ctx: \tm \to \tmtwo$ be a useful step. If $\ctx$ is a $\tolou$ step then $\ctx$ is \lou.
\end{lemma}

\begin{proof}
Properties in the definition of \lou\ contexts:
		\begin{varenumerate}
			\item \emph{Outermost}: if $\ctx = \ctxtwop{\la\var\ctxthree}$ then clearly $\ctxtwo$ is not applicative, otherwise there is a useful redex (the $\todb$ redex involving $\la\var\ctxthree$) containing $\ctx$, \ie\ $\ctx$ is not the \lou\ redex, that is absurd.
			\item \emph{Leftmost}: suppose that the leftmost property of \lou\ contexts is violated for $\ctx$, and let $\ctx = \ctxtwop{\tmthree\ctxthree}$ be such that $\relunf\tmthree\ctxtwo$ is not neutral. We have that $\tmthree$ is $\tolou$-normal. Two cases:
			\begin{varvarenumerate}
			\item \emph{$\relunf\tmthree\ctxtwo$ is an abstraction}. Then $\ctxtwo$ is the position of a useful redex and $\ctx$ is not the \lou\ step, absurd. 
			\item \emph{$\relunf\tmthree\ctxtwo$ contains a $\beta$-redex}. By the contextual normal form property (\reflemma{nf-charac}) there is a useful redex in $\tm$ having its position in $\tmthree$, and so $\ctx$ is not the position of the $\tolou$-redex, absurd.
			\end{varvarenumerate}
		\end{varenumerate}
\end{proof}

\subsection{Inductive \lou\ Contexts} We introduce the alternative characterization of \lou\ contexts, avoiding relative unfoldings. \ben{We call it \emph{inductive} because it follows the structure of the context $\ctx$, even if in the last clause the hypothesis might be  syntactically bigger than the conclusion. Something, however, always decreases: in the last clause it is the number of ES. The lemma that follows is indeed proved by induction over the number of ES in $\ctx$ and $\ctx$ itself.}
 
 \begin{definition}[Inductive \lou\ Contexts]
  A context $\ctx$ is \emph{inductively \lou} (or \ilou), if a judgment about it can be derived by using the following inductive rules:    
  \begin{center}
$\begin{array}{cccccc}
	\AxiomC{}
	\RightLabel{(ax-\ilou)}
	\UnaryInfC{$\ctxhole$ is \ilou}
	\DisplayProof
	&
	\AxiomC{$\ctx$ is \ilou}
	\AxiomC{$\ctx\neq\sctxp{\la\var\ctxtwo}$}
	\RightLabel{(@l-\ilou)}
	\BinaryInfC{$\ctx \tm$ is \ilou}
	\DisplayProof \\\\
	
		\AxiomC{$\ctx$ is \ilou}
	\RightLabel{($\l$-\ilou)}
	\UnaryInfC{$\la\var\ctx$ is \ilou}
	\DisplayProof 
	&
		\AxiomC{$\unf\tm$ is neutral}
		\AxiomC{$\ctx$ is \ilou}
		\RightLabel{(@r-\ilou)}
		\BinaryInfC{$\tm \ctx$ is \ilou}
		\DisplayProof 
		 \\\\
	\multicolumn{2}{c}{	  
	\AxiomC{$\ctx\isub\var{\unf\tm}$ is \ilou}
	\RightLabel{(ES-\ilou)}
	\UnaryInfC{$\ctx \esub\var\tm$ is \ilou}
	\DisplayProof
	}
\end{array}$
\end{center}  
 \end{definition}
 
 Let us show that \lou\ contexts are inductive \lou\ contexts.


\begin{lemma}[\lou\ Contexts are \ilou]
  \label{l:ilou-eq-rlou}
 Let $\ctx$ be a context. If $\ctx$ is \lou\ then $\ctx$ is inductively \lou.
\end{lemma}

\begin{proof}
  By lexicographic induction on $(\esmeas\ctx,\ctx)$, where $\esmeas\ctx$ is the number of ES in $\ctx$. Cases of $\ctx$: 
 \begin{varenumerate}
  \item \emph{Empty} $\ctx = \ctxhole$. Immediate.
  
  \item \emph{Abstraction} $\ctx = \la\var\ctxtwo$. By \ih\ $\ctxtwo$ is \ilou. Then $\ctx$ is \ilou\ by rule ($\l$-\ilou).
  
  \item \emph{Left Application} $\ctx = \ctxtwo \tmtwo$. By \ih, $\ctxtwo$ is \ilou. Note that $\ctxtwo \neq \sctxp{\la\var\ctxthree}$ otherwise the outermost property of \lou\ contexts would be violated, since $\ctxtwo$ appears in an applicative context. Then $\ctx$ is \ilou\ by rule (@l-\ilou).
  
  \item \emph{Right Application} $\ctx = \tmtwo \ctxtwo$. Then $\ctxtwo$ is \lou\ and so $\ctxtwo$ is \ilou\ by \ih. By the leftmost property of \lou\ contexts $\unf\tmtwo = \relunf\tmtwo\ctxhole$ is neutral. Then  $\ctx$ is \ilou\ by rule (@r-\ilou).
  
  \item \emph{Substitution} $\ctx = \ctxtwo\esub\var\tmtwo$. We  prove that $\ctxtwo\isub\var{\unf\tmtwo}$ is \lou\ and obtain that $\ctx$ is \ilou\ by applying the \ih\ (first component decreases) and rule (ES-\ilou). There are two conditions to check:
    \begin{varvarenumerate}
     \item \emph{Outermost}: consider $\ctxtwo\isub\var{\unf\tmtwo} = \ctxthreep{\la\vartwo\ctxfour}$.  Note that the abstraction $\l\vartwo$ comes from an abstraction of $\ctxtwo$ to which $\isub\var{\unf\tmtwo}$ has been applied, because $\unf\tmtwo$ cannot contain a context hole. Then $\ctxtwo = \ctx_2\ctxholep{\la\vartwo\ctx_3}$ with $\ctx_2\isub\var{\unf\tmtwo} =\ctxthree$ and $ \ctx_3\isub\var{\unf\tmtwo} =\ctxfour$. By hypothesis $\ctx$ is \lou\ and so $\ctx_2\esub\var{\unf\tmtwo}$ is not applicative. Then $\ctx_2$ and thus $\ctx_2\isub\var{\unf\tmtwo}$ are not applicative.
     
     \item \emph{Leftmost}: consider $\ctxtwo\isub\var{\unf\tmtwo} = \ctxthreep{\tmthree\ctxfour}$. Note that the application $\tmthree\ctxfour$ comes from an application of $\ctxtwo$ to which $\isub\var{\unf\tmtwo}$ has been applied, because $\unf\tmtwo$ cannot contain a context hole. Then  $\ctxtwo = \ctx_2\ctxholep{\tmthree'\ctx_3}$ with $\ctx_2\isub\var{\unf\tmtwo} =\ctxthree$, $\tmthree'\isub\var{\unf\tmtwo} = \tmthree$, and $ \ctx_3\isub\var{\unf\tmtwo} =\ctxfour$. We have to show that $\relunf\tmthree\ctxthree$ is neutral. Note that 
	
     \begin{center}
      $\relunf\tmthree\ctxthree = \relunf{\tmthree'\isub\var{\unf\tmtwo}}{\ctx_2\isub\var{\unf\tmtwo}} =_{\reflemmaeqp{relunf-prop}{four}} \relunf{\tmthree'}{\ctx_2\esub\var{\tmtwo}}$
     \end{center}
     Since $\ctx = \ctx_2\ctxholep{\tmthree'\ctx_3}\esub\var{\tmtwo}$ is \lou\ by hypothesis, we obtain that $\relunf{\tmthree'}{\ctx_2\esub\var{\tmtwo}}$ is neutral.
    \end{varvarenumerate}
 \end{varenumerate}
\end{proof}

\subsection{Unfolding \lou\ steps} Finally, we show that inductive \lou\ contexts unfold to inductive \lob\ contexts (\refdef{ilob-ctx}, page \pageref{def:ilob-ctx}).

\begin{lemma}[\ilou\ unfolds to \ilob]
	\label{l:useful-projection}
If $\ctx$ is an \ilou\ context then $\unf\ctx$ is a \ilob\ context.
\end{lemma}

\begin{proof}
%By \reflemma{loudb-are-ilou}, the context $\ctx$ of a $\tolou$ $\db$-redex is \lou. By \reflemma{ilou-eq-rlou}, $\ctx$ is also \ilou.

By lexicographic induction on $(\esmeas\ctx,\ctx)$. Cases of $\ctx$. 
 	\begin{varenumerate}
		\item \emph{Empty} $\ctx = \ctxhole$. Then $\unf\ctx = \unf\ctxhole = \ctxhole$ is \ilob.
		\item \emph{Abstraction} $\ctx = \la\var \ctxtwo$. By definition of unfolding $\unf\ctx = \la\var\unf\ctxtwo$, and by the \ilou\ hypothesis $\ctxtwo$ is \ilou. Then by \ih\ (second component), $\unf\ctxtwo$ is \ilob, and so $\unf\ctx$ is \ilob\ by rule ($\l$-\ilob).
		\item \emph{Left Application} $\ctx = \ctxtwo \tm$. By definition of unfolding, $\unf\ctx = \unf\ctxtwo \unf\tm$, and by the \ilou\ hypothesis $\ctxtwo$ is \ilou. Then by \ih\ (second component), $\unf\ctxtwo$ is \ilob. Moreover, $\ctxtwo\neq\sctxp{\la\var\ctxthree}$, that implies $\ctxtwo=\sctxp{\ctxthree\tmtwo}$, $\ctxtwo=\sctxp{\tmtwo\ctxthree}$, or $\ctxtwo=\sctx$. In all such cases we obtain $\unf\ctxtwo\neq \la\var\gctx$. Therefore, $\unf\ctx$ is \ilob\ by rule (@l-\ilob).
		\item \emph{Right Application} $\ctx = \tm \ctxtwo$. By definition of unfolding $\unf\ctx = \unf\tm \unf\ctxtwo $, and by the \ilou\ hypothesis $\ctxtwo$ is \ilou\ and $\unf\tm$ is neutral. Then by \ih\ (second component), $\ctxtwo$ is \ilob, and so $\ctx$ is \ilob\ by rule (@r-\ilob).
  		\item \emph{Substitution} $\ctx = \ctxtwo\esub\var\tm$. By definition of unfolding $\unf\ctx = \unf\ctxtwo\isub\var{\unf\tm}$, and by the \ilou\ hypothesis $\ctxtwo\isub\var{\unf\tm}$ \ilou. Then by \ih\ (first component) $\unf{\ctxtwo\isub\var{\unf\tm}}$ is \ilob, that is equivalent to the statement because $\unf\ctxtwo\isub\var{\unf\tm} =_{\reflemmaeqp{relunf-prop}{zero}} \unf{\ctxtwo\isub\var{\unf\tm}}$.
  	\end{varenumerate}
\end{proof}

The projection property of \lou\ $\todb$ steps now follows easily:

\begin{theorem}[Strong Projection Property]
	\label{tm:projection}
	Let $\tm$ be a \lsc\ term and $\tm\tolou\tmtwo$ a $\todb$ step. Then $\unf{\tm}\toblo\unf{\tmtwo}$.
\end{theorem}


\begin{proof}
	 $\tolou$-steps take place in \lou\ contexts (\reflemma{loudb-are-ilou}), \lou\ contexts are inductive \lou\ contexts (\reflemma{ilou-eq-rlou}), that unfold to \ilob\ contexts (\reflemma{useful-projection}), which is where $\toblo$ steps take place (\reflemma{toblo-ilob}).
\end{proof}

\ben{The following corollary shows that in fact for our high-level implementation system the converse statements of the normal form and projection properties are also valid, even if they are not needed for the invariance result.

\begin{corollary}
\label{c:converse-prop-high-lev}\hfill % \reflemmap{converse-prop-high-lev}{normal}
 \begin{varenumerate}
  \item \label{p:converse-prop-high-lev-normal}
    \emph{Converse Normal Form}: if $\unf\tm$ is a $\beta$-normal form then
    $\tm$ is a useful normal form.
  \item 
    \emph{Converse Projection}: if $\unf\tm\toblo\tmtwo$ then there exists $\tmthree$ such that $\tm\tolou\tmthree$ with $\unf\tmthree=\unf\tm$ or $\unf\tmthree=\tmtwo$.
\end{varenumerate}
\end{corollary}

\begin{proof}\hfill
 \begin{varenumerate}
  \item Suppose that $\tm$ has a useful redex. By the strong projection property (\reftm{projection}) the $\tolou$ redex  in $\tm$ cannot be a $\db$-redex, otherwise $\unf\tm$ is not $\beta$-normal. Similarly, by \reflemma{useful-prom-on-beta} it cannot be a $\ls$-redex. Absurd.    
  \item By the normal form property (\refcoro{normal-form}) $\tm$ has a useful redex, otherwise $\unf\tm$ is $\beta$-normal, that is absurd. Then the statement follows from the strong projection property (\reftm{projection}) or from \reflemma{ls-unfolding}.    
\end{varenumerate} 
\end{proof}
}

\ben{
For the sake of completeness, let us also point out that the converse statements of \reflemma{loudb-are-ilou} (\ie\ useful steps taking place in \lou\ contexts are $\tolou$ steps) and \reflemma{useful-projection} (inductive \lou\ contexts are \lou\ contexts) are provable. We omitted them to lighten the technical development of the paper.
}


==> unfoldings.tex <==
% !TEX root = main.tex
\section{Unfoldings}
In \refsect{hard}, we defined the unfolding $\unf\tm$ of a term $\tm$
(\refdef{unfolding}, page \pageref{def:unfolding}). Here we extend it
in various ways. We first define context unfoldings, then we
generalize the unfolding (of both terms and contexts) relatively to a
context, and finally we unfold shallow derivations.

\subsection{Unfolding Contexts} Shallowness is crucial here: the
unfolding of a shallow context is still a context, because the hole
cannot be duplicated by unfolding, being out of all ES.  First of all,
we define \emph{substitution on (general) contexts}:
\begin{center}
$\begin{array}{rclllrclllllll}
	\ctxhole\isub\var\tmtwo 			& \defeq & \ctxhole\\
	(\la\vartwo\gctx)\isub\var\tmtwo 	& \defeq & \la\vartwo\gctx\isub\var\tmtwo
	&&&(\la\var\gctx)\isub\var\tmtwo 	& \defeq & \la\var\gctx\\
	(\tm \gctx)\isub\var\tmtwo 			& \defeq & \tm\isub\var\tmtwo \gctx\isub\var\tmtwo
	&&&(\gctx \tm)\isub\var\tmtwo 			& \defeq & \gctx\isub\var\tmtwo \tm\isub\var\tmtwo\\
	\gctx \esub\vartwo\tm\isub\var\tmtwo	& \defeq & \gctx\isub\var\tmtwo \esub\vartwo{\tm\isub\var\tmtwo}
	&&&\gctx \esub\var\tm\isub\var\tmtwo	& \defeq & \gctx\esub\var{\tm\isub\var\tmtwo}\\
	\tm \esub\vartwo\gctx\isub\var\tmtwo	& \defeq & \tm\isub\var\tmtwo \esub\vartwo{\gctx\isub\var\tmtwo}
	&&&\tm \esub\var\gctx\isub\var\tmtwo	& \defeq & \tm \esub\var{\gctx\isub\var\tmtwo}
\end{array}$
\end{center}
\ben{Note that the definition of $\ctx\isub\var\tmtwo$ assumes that the free variables of $\tmtwo$ are not captured by $\ctx$ (that means that for instance $\vartwo\notin\fv\tmtwo$ in $(\la\vartwo\gctx)\isub\var\tmtwo$). This can always be achieved by $\alpha$-renaming $\ctx$ (according to \refrem{alpha-for-contexts})}.

And then define \emph{context unfolding} $\unf\ctx$ as:
\begin{center}
$\begin{array}{lllllllllllll}
	\unf\ctxhole 				& \defeq & \ctxhole
	&&&\unf{(\la\var\ctx)} 		& \defeq & \la\var\unf{\ctx}\\
	\unf{(\tm \ctx)} 		& \defeq & \unf\tm \unf{\ctx}
	&&&\unf{(\ctx \tm)} 		& \defeq & \unf{\ctx} \unf\tm\\
	\unf{\ctx \esub\var\tm} 		& \defeq & \unf\ctx \isub\var{\unf\tm}
\end{array}$
\end{center}
We have the following properties.
\begin{lemma}
\label{l:ctx-unf-new} % \reflemmap{ctx-unf-new}{two}
Let $\ctx$ be a shallow contexts. Then:
\begin{varenumerate}
\item\label{p:ctx-unf-new-one}
  $\unf{\ctx}$ is a context;
\item\label{p:ctx-unf-new-two}
  $\ctxp\tm\isub\var\tmtwo={\ctx\isub\var\tmtwo}\ctxholep{\tm\isub\var\tmtwo}$;
\end{varenumerate}
\end{lemma}
\begin{proof}
  By induction on $\ctx$.
\end{proof}

An important notion of context will be that of applicative context,
\ie\ of context whose hole is applied to an argument, and that if
plugged with an abstraction provides a $\db$-redex.
\begin{definition}[Applicative Context]
\label{def:ap-context}
An \deff{applicative context} is a context $\apctx \grameq
\ctxp{\sctx\tm}$, where $\ctx$ and $\sctx$ are a shallow and a
substitution context, respectively.
\end{definition}
Note that applicative contexts are \emph{not} made out of applications
only: $\tm (\l \var.(\ctxhole \esub\vartwo\tmtwo \tmthree))$ is an
applicative context.

\begin{lemma}
\label{l:ap-unf} % \reflemmap{ap-unf}{unf}
Let $\ctx$ be a context. Then,
 \begin{varenumerate}
  \item\label{p:ap-unf-sub} $\ctx$ is applicative iff $\ctx\isub\var\tm$ is applicative;
  \item\label{p:ap-unf-unf}
  $\ctx$ is applicative iff $\unf\ctx$ is applicative.
 \end{varenumerate} 
\end{lemma}

\subsection{Relative Unfoldings}

\ben{Useful reduction will require a more general notion of unfolding
  and context unfolding. The usefulness of a redex, in fact, will
  depend crucially on the context in which it takes place. More
  precisely, it will depend on the unfolding of the term extended with
  the substitutions that the surrounding context can provide---this is
  the unfolding of a term \emph{relative to} a context. Moreover, relative
  unfoldings will also be needed for contexts.}

\begin{definition}[Relative Unfolding]
\ben{Let $\ctx$ be a (shallow) context (verifying, as usual, Barendregt's convention---see also the remark after this definition)}. The \emph{unfolding
$\relunf{\tm}{\ctx}$ of a term $\tm$ relative to $\ctx$} and the \emph{unfolding
$\relunf{\ctxtwo}{\ctx}$ of a (shallow) context $\ctxtwo$ relative to $\ctx$} are defined by:

\begin{center}
\begin{tabular}{cccccccc}
$\begin{array}{lllllllllllll}
	\relunf\tm\ctxhole 				& \defeq & \unf\tm\\
	\relunf\tm{\la\var\ctx} 		& \defeq & \relunf\tm \ctx\\
	\relunf\tm{\tmtwo \ctx} 		& \defeq & \relunf\tm \ctx\\
	\relunf\tm{\ctx \tmtwo} 		& \defeq & \relunf\tm\ctx\\
	\relunf\tm{\ctx \esub\var\tmtwo} 		& \defeq & \relunf{\tm}{\ctx} \isub\var{\unf\tmtwo}
\end{array}$ &&&&&

$\begin{array}{lllllllllllll}
	\relunf\ctxtwo\ctxhole 				& \defeq & \unf\ctxtwo\\
\relunf\ctxtwo{\la\var\ctx} 		& \defeq & \relunf\ctxtwo \ctx\\
	\relunf\ctxtwo{\tmtwo \ctx} 		& \defeq & \relunf\ctxtwo \ctx\\
	\relunf\ctxtwo{\ctx \tmtwo} 		& \defeq & \relunf\ctxtwo\ctx\\
	\relunf\ctxtwo{\ctx \esub\var\tmtwo} 		& \defeq & \relunf{\ctxtwo}{\ctx} \isub\var{\unf\tmtwo}
\end{array}$
\end{tabular}
\end{center}
\end{definition}
For instance, $\relunf{(\ap\var\vartwo)}{(\ap{\ctxhole\esub\vartwo\var}\tm)\esub\var{\l\varthree.(\ap\varthree\varthree)}}
  =
  {(\l\varthree.(\ap\varthree\varthree))}{(\l\varthree.(\ap\varthree\varthree))}$. 
\ben{  
  \begin{remark}[Relative Unfoldings and Barendregt's Convention]
   Let us point out that the definition of relative unfolding $\relunf\tm\ctx$ relies crucially on the use of Barendregt's convention for contexts (according to \refrem{alpha-for-contexts}). For contexts not respecting the convention, in fact, the definition does not give the intended result. For instance, 
   $$\relunf\var{(\la\var\ctxhole)\esub\var\vartwo} = \relunf\var{(\la\var\ctxhole)}\isub\var\vartwo = \relunf\var\ctxhole \isub\var\vartwo = \var\isub\var\vartwo = \vartwo$$
   while the result should clearly be $\var$.
  \end{remark}
  }
  We also state some further properties of relative unfolding, to be used in the proofs, and proved by easy inductions.

\begin{lemma}[Properties of Relative Unfoldings]
	\label{l:relunf-prop} % \reflemmaeqp{relunf-prop}{zero}
	Let $\tm$ and $\tmtwo$ be terms and $\ctx$ and $\ctxtwo$ be shallow contexts.
	\begin{varenumerate}
		\item \label{p:relunf-prop-minusone} \emph{Well-Definedness}: $\relunf{\ctx}\ctxtwo$ is a context.
		
		\item \label{p:relunf-prop-zero} \emph{Commutation}: the following equalities hold \ben{(and in those on the right $\ctx$ is assumed to not capture $\var$)}
		
		\begin{center}$\begin{array}{rclccrcl}
		 \relunf{(\tm\tmtwo)}\ctx   	& = & \relunf\tm\ctx \relunf\tmtwo\ctx
		 &&& \relunf{(\la\var\tm)}\ctx  	& = & \relunf{\la\var\tm}\ctx\\
		 \relunf{\tm\isub\var\tmtwo}\ctx & = & \relunf{\tm\esub\var\tmtwo}\ctx
		 &&& \relunf{\tm\isub\var\tmtwo}\ctx & = & \relunf\tm\ctx \isub\var{\relunf\tmtwo\ctx}\\
		 \unf\ctx\isub{\var}{\unf\tm} 	& = & \unf{\ctx\isub{\var}{\unf\tm}}
		 &&& \relunf\tm{\ctx\esub\var\tmtwo} & = & \relunf{\tm\isub\var{\unf\tmtwo}}{\ctx\isub\var{\unf\tmtwo}}
		\end{array}$\end{center}

		\item \label{p:relunf-prop-one} \emph{Freedom}:
		if $\ctx$ does not capture any free variable of $\tm$ then $\relunf\tm\ctx = \unf\tm$.
		
		\item \label{p:relunf-prop-five} \emph{Relativity}:
		if $\unf\tm =\unf\tmtwo$ then $\relunf\tm\ctx = \relunf\tmtwo\ctx$ and if $\unf\tm$ has a $\beta$-redex then so does $\relunf\tm\ctx$.
		
		\item \label{p:relunf-prop-six} \emph{Splitting}:
		$ \relunf\tm{\ctxp\ctxtwo} = \relunf{\relunf\tm\ctxtwo}{\ctx}$.
		
		\item \label{p:relunf-prop-four} \emph{Factorization}:
		$ \relunf{\ctxtwop\tm}\ctx = \relunf\ctxtwo\ctx \ctxholep{\relunf\tm{\ctxp\ctxtwo}}$, and in particular 
		\begin{varvarenumerate}
		 \item \label{p:relunf-prop-four-a}$ \unf{\ctxp\tm} = \unf\ctx \ctxholep{\relunf\tm{\ctx}}$,
		 \item $ \relunf{\sctxp\tm}\ctx = \relunf\tm{\ctxp\sctx}$, and
		 \item if $\ctxtwo\prefix\tmtwo$ then $\unf{\ctxtwo}\prefix\unf{\tmtwo}$.
		\end{varvarenumerate}

	\end{varenumerate}
\end{lemma}

\subsection{Unfolding Derivations}
Given a derivation $\deriv:\tm\to^*\tmtwo$ in the \lsc, we often
consider the $\beta$-derivation
$\unf{\deriv}:\unf{\tm}\tob^*\unf{\tmtwo}$ obtained by projecting
$\deriv$ via unfolding. It is built in two steps.

As expected, linear substitution steps do not modify the unfolding, as the next lemma shows. \ben{Its proof is a nice application of the properties of contexts and (relative) unfoldings, allowed by the restriction to shallow contexts (the property is valid more generally for unrestricted $\ls$ steps, but we will need it only for the shallow ones).}

\begin{lemma}[$\tols$ Projects on $=$]
\label{l:ls-unfolding}
 If $\tm\tols\tmtwo$ then $\unf\tm = \unf\tmtwo$.
\end{lemma}

\ben{
\begin{proof}
 If $\tm \tols\tmtwo$ is a root step, \ie\ $\tm = \ctxp\var \esub\var\tmthree \rtols \ctxp\tmthree \esub\var\tmthree = \tmtwo$ then 
 \[\begin{array}{rllclc}
    \unf{\ctxp\var \esub\var\tmthree} & = & \unf{\ctxp\var} \isub\var{\unf\tmthree} \\
    & =_\reflemmaeqp{relunf-prop}{four-a} & \unf\ctx\ctxholep{\relunf\var\ctx} \isub\var{\unf\tmthree} \\
    & =_\reflemmaeqp{relunf-prop}{one} & \unf\ctx\ctxholep\var \isub\var{\unf\tmthree} \\
    & =_\reflemmaeqp{ctx-unf-new}{two} & \unf\ctx\isub\var{\unf\tmthree}\ctxholep{\unf\tmthree} \\
    & = & \unf\ctx\isub\var{\unf\tmthree}\ctxholep{\unf\tmthree\isub\var{\unf\tmthree}} \\
    & =_\reflemmaeqp{ctx-unf-new}{two} & \unf\ctx\ctxholep{\unf\tmthree}\isub\var{\unf\tmthree} \\
    & =_\reflemmaeqp{relunf-prop}{one} & \unf\ctx\ctxholep{\relunf\tmthree\ctx}\isub\var{\unf\tmthree} \\
    & =_\reflemmaeqp{relunf-prop}{four-a} & \unf{\ctxp\tmthree}\isub\var{\unf\tmthree}  \\
    & = & \unf{\ctxp\tmthree \esub\var\tmthree}
    \end{array}\]
 Suppose instead $\tm \tols\tmtwo$ because $\tm = \ctxtwop\tmthree \tols \ctxtwop\tmfour = \tmtwo$ with $\tmthree\rtols\tmfour$. By what we just proved we obtain $\unf\tmthree = \unf\tmfour$, that gives $\relunf\tmthree\ctxtwo = \relunf\tmfour\ctxtwo$ by \reflemmap{relunf-prop}{five}. Then $\unf{\ctxtwop\tmthree} =_\reflemmaeqp{relunf-prop}{four-a} = \unf\ctxtwo\ctxholep{\relunf\tmthree\ctxtwo} = \unf\ctxtwo\ctxholep{\relunf\tmfour\ctxtwo} =_\reflemmaeqp{relunf-prop}{four-a} = \unf{\ctxtwop\tmfour}$.
\end{proof}
}

Instead, $\db$-steps project to $\beta$-steps. Because of shallowness, we actually obtain a strong form of projection, as every $\db$-step projects on a single $\beta$-step. We are then allowed to identify $\db$ and $\beta$-redexes. 

\begin{lemma}[$\todb$ Strongly Projects on $\tob$]
	\label{l:db-projection}
	Let $\tm$ be a \lsc\ term and $\ctx:\tm\todb\tmtwo$ a $\db$-redex in $\tm$. Then $\unf\ctx: \unf\tm\tob\unf\tmtwo$.
	
\end{lemma}

\begin{proof} 

Let $\tm=\ctxp {\tmthree}\todb\ctxp{\tmfour}=\tmtwo$ with $\tmthree\rtodb\tmfour$. We show that $\unf{\ctx}:\unf{\tm}=\unf{\ctx}\ctxholep{\relunf{\tmthree}{\ctx}}\tob\unf{\ctx}\ctxholep{\relunf{\tmfour}{\ctx}}=\unf{\tmtwo}$ with $\relunf{\tmthree}{\ctx}\rtob\relunf{\tmfour}{\ctx}$ ($\rtodb$ and $\rtob$ stands for $\db/\beta$-reduction at top level). By induction on $\ctx$. Cases:
\begin{varenumerate}
	\item \emph{Empty context $\ctx=\ctxhole$}. Notation: given $\sctx=\esub{\var_1}{\tmthree_1}\ldots\esub{\var_n}{\tmthree_n}$ we denote with $\sctximp$ the list of implicit substitutions $\isub{\var_1}{\tmthree_1}\ldots\isub{\var_n}{\tmthree_n}$.  Then $\tm=\tmthree=\sctxp{\l\var.\tmfive}\tmsix$, $\unf{\tm}=\relunf{\tmthree}{\ctx} = \unf\tmthree$, $\tmtwo=\tmfour$, $\unf{\tmtwo}=\relunf{\tmfour}{\ctx} = \unf\tmfour$, and
		\begin{center}
			\commDiagramRed{$\tm=\sctxp{\l\var.\tmfive}\tmsix$            }{
											$\sctxp{\tmfive\esub\var\tmsix}=\tmtwo$		       }{
											$\unf{\tm}=(\l\var.\unf{\tmfive}\sctximp) (\unf{\tmsix})   $}{
											$\unf{\tmfive}\sctximp \isub\var{\unf{\tmsix}}=\unf{\tmfive}\isub\var{\unf{\tmsix}}\sctximp   =\unf{\tmtwo}$ }{
											$\db$}{$\beta$}{\unfsym}{\unfsym}
		\end{center}
		where the first equality in the South-East corner is given by the fact that $\var$ does not occur in $\sctx$ and the variables on which $\sctximp$ substitutes do not occur in $\tmsix$, as is easily seen by looking at the starting term. Thus the implicit substitutions $\sctximp$ and $ \isub\var{\unf{\tmsix}}$ commute.
		
		
	\item \emph{Abstraction $\ctx=\l\var.\ctxtwo$}. It follows immediately by the \ih
	
	\item \emph{Left of an application $\ctx=\ctxtwo\tmfive$}. By \reflemmap{relunf-prop}{zero} we know that $\unf{\tm}=\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}\unf{\tmfive}$. Using the \ih\ we derive the following diagram:		
		\begin{center}
			\commDiagramRed{$
											\ctxtwop\tmthree\tmfive
											$}{$
											\ctxtwop\tmfour\tmfive
											$}{$
											\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}\unf{\tmfive}
											$}{$
											\unf{\ctxtwo}\ctxholep{\relunf{\tmfour}{\ctxtwo}}\unf{\tmfive}
											$}{$
											\db$}{$\beta$}{\unfsym}{\unfsym}
		\end{center}

\item \emph{Right of an application $\ctx=\tmfive\ctxtwo$}. By \reflemmap{relunf-prop}{zero} we know that $\unf{\tm}=\unf{\tmfive}\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}$. Using the \ih\ we derive the following diagram:		
		\begin{center}
			\commDiagramRed{$
											\tmfive\ctxtwop\tmthree
											$}{$
											\tmfive\ctxtwop\tmfour
											$}{$
											\unf{\tmfive}\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}
											$}{$
											\unf{\tmfive} \unf{\ctxtwo}\ctxholep{\relunf{\tmfour}{\ctxtwo}}
											$}{$
											\db$}{$\beta$}{\unfsym}{\unfsym}
		\end{center}
	\item \emph{Substitution $\ctx=\ctxtwo\esub\var\tmfive$}. By \ih\ $\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}\tob \unf{\ctxtwo}\ctxholep{\relunf{\tmfour}{\ctxtwo}}$ with $\relunf{\tmthree}{\ctxtwo} \rtob \relunf{\tmfour}{\ctxtwo}$. In general, from the definition of substitution it follows $\tmsix\rtob\tmsix'$ implies $\tmsix\isub\var{\tmsix''}\rtob\tmsix'\isub\var{\tmsix''}$. Therefore, $\relunf{\tmthree}{\ctxtwo}\isub\var{\unf\tmfive} \rtob \relunf{\tmfour}{\ctxtwo}\isub\var{\unf\tmfive}$. The following calculation concludes the proof:
$$
\begin{array}{llllllll}
\unf{\tm}&=&
\unf{\ctxtwo}\ctxholep{\relunf{\tmthree}{\ctxtwo}}\isub\var{\unf\tmfive}\\
&=_{\reflemmaeqp{ctx-unf-new}{two}}&\unf{\ctxtwo}\isub\var{\unf\tmfive}\ctxholep{\relunf{\tmthree}{\ctxtwo}\isub\var{\unf\tmfive}}\\
&\tob &\unf{\ctxtwo}\isub\var{\unf\tmfive}\ctxholep{\relunf{\tmfour}{\ctxtwo}\isub\var{\unf\tmfive}}\\
&=_{\reflemmaeqp{ctx-unf-new}{two}}&\unf{\ctxtwo}\ctxholep{\relunf{\tmfour}{\ctxtwo}}\isub\var{\unf\tmfive}\unf{\tmtwo}
\end{array}
$$
\end{varenumerate}
\end{proof}

% The following theorem follows from \reflemma{ls-unfolding} ($\tols$ projects on =) and \reflemma{db-projection} ($\todb$ projects on $\tob$).
% 
% \begin{theorem}[Shallow Projection]
% \label{thm:shal-proj}
% Let $\deriv:\tm\to^*\tmtwo$ be a derivation. Then $\unf\deriv:\unf\tm\tob^*\unf\tmtwo$ with $\size{\unf\deriv} = \sizedb\deriv$.
% \end{theorem}

